Consistent and Efficient MSCKF-based LiDAR-Inertial Odometry with Inferred Cluster-to-Plane Constraints for UAVs

Robust and accurate navigation is critical for Unmanned Aerial Vehicles (UAVs) especially for those with stringent Size, Weight, and Power (SWaP) constraints. However, most state-of-the-art (SOTA) LiDAR-Inertial Odometry (LIO) systems still suffer from estimation inconsistency and computational bottlenecks when deployed on such platforms. To address these issues, this paper proposes a consistent and efficient tightly-coupled LIO framework tailored for UAVs. Within the efficient Multi-State Constraint Kalman Filter (MSCKF) framework, we build coplanar constraints inferred from planar features observed across a sliding window. By applying null-space projection to sliding-window coplanar constraints, we eliminate the direct dependency on feature parameters in the state vector, thereby mitigating overconfidence and improving consistency. More importantly, to further boost the efficiency, we introduce a parallel voxel-based data association and a novel compact cluster-to-plane measurement model. This compact measurement model losslessly reduces observation dimensionality and significantly accelerating the update process. Extensive evaluations demonstrate that our method outperforms most state-of-the-art (SOTA) approaches by providing a superior balance of consistency and efficiency. It exhibits improved robustness in degenerate scenarios, achieves the lowest memory usage via its map-free nature, and runs in real-time on resource-constrained embedded platforms (e.g., NVIDIA Jetson TX2).

==> proof.tex <==

\section{Proof of Lemma~\ref{lemma:equivalence}}
\label{sec:proof1}

% \begin{proof}
% proof: 首先，卡尔曼滤波的更新过程可以被写为如下形式：
The update process of the Kalman filter can be expressed as follows.

The expression for obtaining the Kalman gain is given by:
\begin{equation}
    \mathbf{K} =  (\hat{\mathbf{P}}^{-1} + \mathbf{H}^T\mathbf{R}^{-1}\mathbf{H})^{-1}\mathbf{H}^T\mathbf{R}^{-1}
\end{equation}
% 这种卡尔曼增益的计算方式与标准卡尔曼增益计算方式完全等价，可参考fastlio.
This computation method for the Kalman gain is strictly equivalent to the standard Kalman gain formulation, as formally established in\cite{xu2021fast, jahja2019kalman}.

The posterior update of the state is given by:
\begin{equation}
    \bar{\mathbf{X}} = \bm K \bm Z = (\hat{\mathbf{P}}^{-1} + \mathbf{H}^T\mathbf{R}^{-1}\mathbf{H})^{-1}\mathbf{H}^T\mathbf{R}^{-1}\bm Z
\end{equation}



The update of the state covariance is given by:
\begin{equation}
    \begin{aligned}
            \bar{\bm P} &= \bm{(I - KH)}\hat{\bm {P}}\\
 &= (\bm I -  (\hat{\mathbf{P}}^{-1} + \mathbf{H}^T\mathbf{R}^{-1}\mathbf{H})^{-1}\mathbf{H}^T\mathbf{R}^{-1}\mathbf{H})\hat{\bm P}
    \end{aligned}
\end{equation}

Therefore, demonstrating that the terms $HR^{-1}H$ and $HR^{-1}Z$ are identical for both observation strategies suffices to prove that the updated state $X$ and covariance $P$ are identical after the Kalman update, thereby establishing the strict equivalence between the two update methods.



% 对于点面残差，其中Z和H 可以写为： 
\textbf{For the residual of point-to-plane observation}, 
The point-to-plane measment $Z$ can be expressed as:
% \begin{equation}
%     % \begin{aligned}
%         
%          % 

%     % \end{aligned}
% \end{equation}
\begin{equation}
    \begin{aligned}
         \bm{Z} &=  \begin{bmatrix} \mathbf{n}^T&-\mathbf{d} \end{bmatrix} \cdot \mathbf{T} \cdot  \begin{bmatrix} \mathbf{p} \\ 1 \end{bmatrix} \\
         &= \begin{bmatrix} \mathbf{p}^T&1 \end{bmatrix} \cdot \mathbf{T}^T  \begin{bmatrix} \mathbf{n} \\ -\mathbf{d} \end{bmatrix}
    \end{aligned}
\end{equation}
% 由于点面残差Z是标量，所以它的转置等于它自身。
Since the point-to-plane residual $\bm Z$ is a scalar, its transpose equals itself.
% 对一位姿T观测到的平面pi上的所有的点形成的点面残差，可以叠加形成如下形式：

The point-to-plane residuals formed by all points on plane $\pi$ observed at pose $T$ can be stacked into the following form: 
\begin{equation}
\bm{Z} = \begin{bmatrix} Z_1\\Z_2\\Z_3\\ \vdots  \\Z_n\end{bmatrix}= \begin{bmatrix} p_1&1\\p_2&1\\p_3&1\\ \vdots& \vdots  \\p_n&1\end{bmatrix} \cdot \mathbf{T}^T \cdot \begin{bmatrix} \mathbf{n} \\ -\mathbf{d} \end{bmatrix}
\end{equation}

% 其对位姿的雅可比矩阵H为：
Its Jacobian matrix  with respect to the pose $T$ is:
\begin{equation}
\bm{H} = \begin{bmatrix} p_1&1\\p_2&1\\p_3&1\\ \vdots& \vdots  \\p_n&1\end{bmatrix} \cdot \begin{bmatrix} (R^Tn)^\wedge &0 \\0 &n^T
\end{bmatrix}
\end{equation}

% 对于该观测
For this measurement
\begin{multline}
\bm{H R^{-1} H}
= \frac{1}{\sigma^2}
\begin{bmatrix}(R^Tn)^\wedge & 0 \\ 0 & n^T\end{bmatrix}^T
\begin{bmatrix}p_1&\dots&p_n\\1&\dots&1\end{bmatrix}\\
\times
\begin{bmatrix}p_1&1\\\vdots&\vdots\\p_n&1\end{bmatrix}
\begin{bmatrix}(R^Tn)^\wedge & 0 \\ 0 & n^T\end{bmatrix}
\end{multline}


\begin{multline}
  \bm{H R^{-1} Z} = \frac{1}{\sigma^2}
  \begin{bmatrix}(R^T n)^\wedge & 0 \\ 0 & n^T\end{bmatrix}^T
  \begin{bmatrix} p_1 & \dots & p_n \\ 1 & \dots & 1 \end{bmatrix} \\
  \times
  \begin{bmatrix} p_1 & 1 \\ \vdots & \vdots \\ p_n & 1 \end{bmatrix}
  \cdot \mathbf{T}^T \cdot
  \begin{bmatrix}\mathbf{n} \\ -\mathbf{d}\end{bmatrix}
\end{multline}

% 对于点簇到平面的观测残差
\textbf{For the residual of point cluster to plane observation:}
\begin{equation}
\bm{Z} = \mathbf{L}^T\cdot \mathbf{T}^T \cdot
\begin{bmatrix}\mathbf{n} \\ -\mathbf{d}\end{bmatrix}
\end{equation}
\begin{equation}
\bm{H} = \mathbf{L}^T\cdot \begin{bmatrix} (R^Tn)^\wedge &0 \\0 &n^T\end{bmatrix}
\end{equation}
% 令R=sigma
Let $R=\frac{1}{\sigma}\cdot\mathbf{I}_{4\times4}$

{\small
\begin{equation}
\bm{HR^{-1}H} = \frac{1}{\sigma^2}\cdot \begin{bmatrix} (R^Tn)^\wedge &0 \\0 &n^T\end{bmatrix}^T \cdot\mathbf{L}\cdot\mathbf{L}^T \cdot 
\begin{bmatrix} (R^Tn)^\wedge &0 \\0 &n^T\end{bmatrix}
\end{equation}
}

\begin{equation}
\bm{HR^{-1}Z} = \frac{1}{\sigma^2}\cdot \begin{bmatrix} (R^Tn)^\wedge &0 \\0 &n^T\end{bmatrix}^T \cdot\mathbf{L}\cdot\mathbf{L}^T \cdot \mathbf{T}^T  \cdot
\begin{bmatrix}\mathbf{n} \\ -\mathbf{d}\end{bmatrix}
\end{equation}

% 又因为：
Given that
\begin{equation}
\mathbf{L}\cdot\mathbf{L}^T = \begin{bmatrix}
    p_1&\dots&p_n\\1&\dots&1
\end{bmatrix}
\begin{bmatrix} p_1&1\\ \vdots& \vdots  \\p_n&1\end{bmatrix}
\end{equation}

% 可以看到点面观测更新和点簇到平面的观测更新两种方式的 $HR^{-1}H$、$HR^{-1}Z$完全相等，因此两种观测在经过EKF过程后结果完全等价。
It can be observed that both the point-to-plane observation update and the point cluster-to-plane observation update yield identical $HR^{-1}H$ and $HR^{-1}Z$ terms. Consequently, the two update strategies produce strictly equivalent results after the EKF process.
%
% \end{proof}
